Lucas-Kanade Reloaded: End-to-End Super-Resolution from Raw Image Bursts

This presentation addresses the problem of reconstructing a high-resolution image from multiple lower-resolution snapshots captured from slightly different viewpoints in space and time. Key challenges for solving this problem include (i) aligning the input pictures with sub-pixel accuracy, (ii) handling raw (noisy) images for maximal faithfulness to native camera data, and (iii) designing/learning an image prior (regularizer) well suited to the task. We address these three challenges with a hybrid algorithm building on the insight from Wronski et al. that aliasing is an ally in this setting, with parameters that can be learned end to end, while retaining the interpretability of classical approaches to inverse problems. The effectiveness of our approach is demonstrated on synthetic and real image bursts, setting a new state of the art on several benchmarks and delivering excellent qualitative results on real raw bursts captured by smartphones and prosumer cameras.

==> notes/degradation_model.tex <==
\subsection{Degradation Model}

\paragraph{Continuous Image Formation Model}

We model the image formation process when shooting a burst of $\{1, \cdots, K\}$ frames with a digital camera. Let $f:\mathbb{R}^2\rightarrow \mathbb{R}$ be the continuous image obtained by an ideal projection of a 3-D scene onto the 2-D image plane of a digital camera (it can then be seen as an image of infinite spatial resolution). In what follows we study  the acquisition process for each color channel (rgb) of the digital camera independently.

\paragraph{Motion model}

The ideal image $f(\ub)$ is assumed to be warped by a geometric
transformation, to describe the acquisition the images sequence. This geometric transformation encodes camera motion between each frame, object motion or a combination of these movements. For the sake of clarity, motion is described on the 2-D image plane.
% \paragraph{Image blur}
% The ideal image model for the frame $g^{(k)}$ of the image burst can be written:
When acquiring the k-th frame of the burst, the camera’s sensor accumulates photons while the shutter is open, and outputs an observed image $g^{(k)}:\mathbb{R}^2\rightarrow \mathbb{R}$ which can be written as:
\begin{equation}
  g^{(k)}(\ub) = \int_{t=t_k}^{t_k+\tau_k} f(M_t(\ub)) * h_{\mathrm{optics}}(\ub) \, dt,
\end{equation}
where $M_t : \mathbb{R}^2 \rightarrow \mathbb{R}^2$ denotes the displacement of $f( \ub )$ at position $\ub$ relative to the reference frame.
% It encodes the motion model for the camera at instant $t$.
% $M_t:\mathbb{R}^2 \rightarrow \mathbb{R}^2$ denotes the movement of the camera through time.
The optical blur $h_\mathrm{optics}(\xb)$ accounts for various corruption phenomena including atmospheric blur, out-of-focus blur, lens diffraction, lens defects.
% It has a dependence on $\xb$ due to the out-of focus blur.

\paragraph{Sampling} Continuous image cannot be processed on digital devices. The only accessible information regarding a set of acquired images are the sampled intensity values at discrete pixel positions. $\mathcal{D}$ denotes the sampling at the pixel positions and $ \epsilon^{(k)}(\xb)$ is a stochastic signal to model measurement noise. The sampling operator is given by:
\begin{equation}
    \mathcal{D} \left \{  f(\ub) \right \} = \sum_{m=-\infty}^\infty \sum_{n=-\infty}^\infty x(u,v) \delta(u-m\delta u,v-m\delta v).
\end{equation}
The convolution with $h_\mathrm{sensor}$ models non ideal sampling due to the integration of light over a finite area on the sensor array corresponding to a pixel of the detector.
The final image formation model is:
\begin{equation}
  y^{(k)}(\ub) = \mathcal{D}_{\mathrm{Bayer}}  \left \{ \int_{t=t_k}^{t_{k+1}} f(M_t(\ub))  * h_\mathrm{optics}(\ub) \, dt * h_{\mathrm{sensor}} \right \}+ \epsilon^{(k)}(\ub),
\end{equation}
where $ \mathcal{D}_{\mathrm{Bayer}}$, denotes the sampling process, relative to the sampling frequency of each color channel (50\% more samples for the green channel than red or blue). 

\paragraph{Discrete Model}
The only accessible information regarding a set of acquired images are the
sampled intensity values at discrete pixel positions.
The intensity values at the pixel positions for each observed frame $y^{(k)}$ are reorganized into a vector of size $\mathbb{R}^{L}$, and $L=L_u L_v$:
\begin{equation}
    \yb = [ f(\Delta u,\Delta v), \cdots, f(L_u \Delta  u,L_v \Delta v)]^\top,
\end{equation}
where $\Delta_u$ and $\Delta_v$ denote the pixel pitch in u- and v-direction, respectively.

\paragraph{Virtual high-quality discrete image}
it is not feasible to reconstruct a continuous representation of the
ideal image $f(\ub)$, we limit ourselves to the reconstruction of a digital image with
finer spatial sampling. By hypothesis the ideal (high-res) digital image $\xb$ results from an ideal sampling of a band-limited signal and therefore does not contain aliasing and is not degraded by any blurring. The spatial resolution  can be chosen arbitrarily.
The samples at pixel position $\ub \in \Omega$ in the image $f(\ub) $ are reorganized to a vector according to
\begin{equation}
    \xb = [ f(\Delta u,\Delta v), \cdots, f(N_u \Delta  u,N_v \Delta v)]^\top.
\end{equation}
$\xb \in \mathbb{R}^{N}$ is referred to as high-resolution image and $N=N_u N_v$.

\paragraph{Discrete formation model}
The image formation from $\xb$ to $\yb$ can be implemented by discrete filter operations:
\begin{equation}
    \yb^{(k)} = \Db \Bb \Wb^{(k)} \xb + \epsilon^{(k)},
\end{equation}
where $\Db \in \mathbb{R}^{L \times M }$ denotes subsampling,  $\Mb \in \mathbb{R}^{M \times N}$ models the subsampling of the Bayer filter,  $\Bb \in \mathbb{R}^{N \times N}$ encodes the blur kernel and  $\Wb \in \mathbb{R}^{N \times N}$ denotes the motion for the k-th frame in matrix
notation. 

